Is Reinforcement Learning More Difficult Than Bandits? A Near-optimal Algorithm Escaping the Curse of Horizon

Episodic reinforcement learning and contextual bandits are two widely studied sequential decision-making problems. Episodic reinforcement learning generalizes contextual bandits and is often perceived to be more difficult due to long planning horizon and unknown state-dependent transitions. The current paper shows that the long planning horizon and the unknown state-dependent transitions (at most) pose little additional difficulty on sample complexity. We consider the episodic reinforcement learning with $S$ states, $A$ actions, planning horizon $H$, total reward bounded by $1$, and the agent plays for $K$ episodes. We propose a new algorithm, \textbf{M}onotonic \textbf{V}alue \textbf{P}ropagation (MVP), which relies on a new Bernstein-type bonus. Compared to existing bonus constructions, the new bonus is tighter since it is based on a well-designed monotonic value function. In particular, the \emph{constants} in the bonus should be subtly setting to ensure optimism and monotonicity. We show MVP enjoys an $O\left(\left(\sqrt{SAK} + S^2A\right) \poly\log \left(SAHK\right)\right)$ regret, approaching the $\Omega\left(\sqrt{SAK}\right)$ lower bound of \emph{contextual bandits} up to logarithmic terms. Notably, this result 1) \emph{exponentially} improves the state-of-the-art polynomial-time algorithms by Dann et al. [2019] and Zanette et al. [2019] in terms of the dependency on $H$, and 2) \emph{exponentially} improves the running time in [Wang et al. 2020] and significantly improves the dependency on $S$, $A$ and $K$ in sample complexity.

==> abs.tex <==
\iffalse
Episodic reinforcement learning and contextual bandits are two widely studied sequential decision-making problems.
Episodic reinforcement learning generalizes contextual bandits and is often perceived to be more difficult due to long planning horizon and unknown state-dependent transitions.
The current paper shows that the long planning horizon and the unknown state-dependent transitions (at most) pose little additional difficulty on sample complexity.


We consider the episodic reinforcement learning with $S$ states, $A$ actions,  planning horizon $H$, total reward bounded by $1$, and the agent plays for $K$ episodes.
We propose a new algorithm, \textbf{M}onotonic \textbf{V}alue \textbf{P}ropagation (MVP), which relies on a new Bernstein-type bonus.
The new bonus only requires tweaking the \emph{constants} to ensure optimism and thus is significantly simpler than existing bonus constructions.
We show MVP enjoys an $O\left(\left(\sqrt{SAK} + S^2A\right) \poly\log \left(SAHK\right)\right)$ regret,
  approaching the $\Omega\left(\sqrt{SAK}\right)$ lower bound of \emph{contextual bandits}.
Notably, this result 1) \emph{exponentially} improves the state-of-the-art polynomial-time algorithms by Dann et al. [2019] and Zanette et al. [2019] in terms of the dependency on $H$, and 2) \emph{exponentially} improves the running time in [Wang et al. 2020] and significantly improves the dependency on $S$, $A$ and $K$ in sample complexity.
\fi

Episodic reinforcement learning and contextual bandits are two widely studied sequential decision-making problems.
Episodic reinforcement learning generalizes contextual bandits and is often perceived to be more difficult due to long planning horizon and unknown state-dependent transitions.
The current paper shows that the long planning horizon and the unknown state-dependent transitions (at most) pose little additional difficulty on sample complexity.


We consider the episodic reinforcement learning with $S$ states, $A$ actions,  planning horizon $H$, total reward bounded by $1$, and the agent plays for $K$ episodes.
We propose a new algorithm, \textbf{M}onotonic \textbf{V}alue \textbf{P}ropagation (MVP), which relies on a new Bernstein-type bonus. Compared to existing bonus constructions, the new bonus is tighter since it is based on a well-designed monotonic value function. In particular, the \emph{constants} in the bonus should be subtly setting
to ensure optimism and monotonicity.

We show MVP enjoys an $O\left(\left(\sqrt{SAK} + S^2A\right) \poly\log \left(SAHK\right)\right)$ regret,
  approaching the $\Omega\left(\sqrt{SAK}\right)$ lower bound of \emph{contextual bandits} up to logarithmic terms.
Notably, this result 1) \emph{exponentially} improves the state-of-the-art polynomial-time algorithms by Dann et al. [2019] and Zanette et al. [2019] in terms of the dependency on $H$, and 2) \emph{exponentially} improves the running time in [Wang et al. 2020] and significantly improves the dependency on $S$, $A$ and $K$ in sample complexity.
%Comparing with the $\Omega\left(\sqrt{SA K}\right)$ lower bound of \emph{contextual bandits}, 
%This bound is appraoching 
%1) matches the information theoretical \emph{lower bound of contextual bandit}, $\Omega\left(\sqrt{SAK}\right)$, up to logarithmic factors and a small additive term $S^2A$, 


%
%
%Our results rely on two key technical innovations: 1) a new, simple exploration bonus based on Bernstein bound via tweaking the \emph{constants} to ensure optimism,
%and 2) a recursion-based analysis technique to bound the variance of the estimated value function.
%We believe these new techniques are widely applicable in reinforcement learning problems.
